Characterizing maximal varieties via Bredon cohomology

We obtain a characterization of Maximal and Galois-Maximal $C_2$-spaces (including real algebraic varieties) in terms of $\operatorname{RO}(C_2)$-graded cohomology with coefficients in the constant Mackey functor $\underline{\mathbf{F}}_2$, using the structure theorem of \cite{clover_may:structure_theorem}. Other known characterizations, for instance in terms of equivariant Borel cohomology, are also rederived from this. For the particular case of a smooth projective real variety $V$, equivariant Poincar\'{e} duality from \cite{pedro&paulo:quaternionic_algebraic_cycles} is used to deduce further symmetry restrictions for the decomposition of the $\operatorname{RO}(C_2)$-graded cohomology of the complex locus $V(\mathbf{C})$ given by the same structure theorem. We illustrate this result with some computations, including the $\operatorname{RO}(C_2)$-graded cohomology with $\underline{\mathbf{F}}_2$ coefficients of real $K3$ surfaces.

==> Sections/symmetric_products.tex <==
\section{Bigraded cohomology of equivariant Eilenberg--Mac Lane spaces $K(\underline{\Z},V)$}
\label{sec:cohomology_eilenberg-maclane}


As in the non-equivariant case, Eilenberg--MacLane spaces correspodning to integer coefficients can be obtained by taking the infinite symmetric product of a sphere.
In this way,
%
\[
K(\underline{\Z},V) = SP_\infty S^V,
\]
%
where $V$ is some $C_2$-representation.
As explained in Section \ref{subsec:symmetric_products}, the infinite symmetric product is fileterd by finite symmetric products.
Moreover, $S^V$ is a maximal space, so the results of Franz from Theorem \ref{thm:gamma_products}, as well as the characterisations of Theorem \ref{prop:main_result} and Proposition \ref{prop:main_result_borel}, will play an important role when proving Theorem \ref{thm:eilenberg-maclane_spaces}.


%-----------------------------------------------------------------------------------------------------------------------------------------------
%
%	ZERO CYCLES
%
%-----------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Zero-cycles}
\label{subsec:zero_cycles}

The other main ingredient in the proof of Theorem \ref{thm:eilenberg-maclane_spaces} is the \emph{zero-cycles} of a space.
Exploding the additive properties that exhibit, and by applying the equivariant Dold--Thom theorem of \cite{pedro:equivariant_dold-thom_theorem}, one obtains a convenient splitting for the equivariant homology of the spaces $K(\underline{\Z},V)$.

%The structure theorem will characterise the space of \emph{zero-cycles} of a finite $C_2$-CW complex.
%From now, by a $C$-complex $X$ it is meant a \emph{pointed} $G$-complex $(X,x_0)$.

\begin{defi}[Zero-cycles]
%\label{def:}
Let $\Gamma$ be an Abelian topological group and let $Z$ be a space.
The symbol $\Gamma[Z]$ denotes the free topological Abelian group on $Z$.
Its elements are formal sums of points in $Z$ with coefficients in $\Gamma$, and are referred to as the \emph{zero-cycles} of $Z$ (with coefficients in $\Gamma$).
The space $\Gamma[Z]$ itself is often called the space of \emph{zero-cycles} of $Z$ (with coefficients in $\Gamma$).
\end{defi}

The topology of $\Gamma[Z]$ is not straightforward.
As coefficients are in $\Gamma$, the correct topology seems to be weakest topology with respect to which all homomorphic extensions of continuous maps from $Z$ to topological $\Z[\Gamma]$-modules are continuous (cf.~\cite{sipacheva:free_boolean_groups}).
Then, the natural inclusion $Z\hookrightarrow \Gamma[Z]$ is a topological embedding.

When $(Z,z_0)$ is a pointed space, then $\tilde\Gamma[X]$ denotes the space of reduced zero-cycles of $Z$:
%
\[
\tilde{\Gamma}[Z] = \Gamma[Z] \Big/ \Gamma[z_0],
\]
%
The underlying set the classifying space $B(\Gamma, Z)$ defined by McCord in \cite{mccord:classifying_spaces}.
Therefore, one may give the corresponding topology to $\tilde{\Gamma}[Z]$.

If another group group $G$ were acting on $Z$, then this action would be carried out on $\Gamma[Z]$ by linear extension, and thsi action would pass to $\tilde\Gamma[Z]$.
We are interested in the case $\Gamma=\F_2$ and $G=C_2$.

The structure theorem of \ref{thm:structure_theorem} implies the following decomposition of the zero-cycles of a $C_2$-space.  

\begin{thm}
\label{thm:0-cycles}
For any finite $C_2$-CW complex $X$, there is a decomposition of the space of its reduced zero cycles as
%
\[
\F_2[X] \simeq_{C_2} \left(\bigoplus_{i\in \tilde I} \tilde\F_2[S^{p_i,q_i}]\right)  \oplus \left(\bigoplus_{j\in J} \tilde\F_2[S^{r_j}\wedge (S^{n_j}_a)_+]\right) .
%\oplus \left(\bigoplus_{j\in J} \tilde\F_2[S^{r_j}\wedge (S^0_a)_+]\right)
\]
%
\end{thm}
\begin{proof}
This result is essentially a reformulation of Theorem 6.13 in \cite{clover_may:structure_theorem}.% but using the corresponding spaces representing the equivariant Eilenberg--MacLane spectrum rather than the spectrum itself.

For each shifted copy of $\Mop_2$ in the homology of $X$, the generator $g$ corresponds to the homotopy class of an equivariant map $g:S^{p,q}\to \F_2[X]$,
as
%
\[
H_{p,q}^{C_2}(X;\underline{\F_2}) \cong [S^{p,q},\F_2[X]]_{C_2} = \pi_{p,q}\left(\F_2[X]\right).
\]
% 
Then, $g$ extends to a map $\F_2[S^{p,q}]\to\F_2[X]$, that will also be denoted by the same symbol.

In the case of antipodal spheres things are more subtle.
For each copy of $\Aop_n$, there exist elements $a_i$ which are annihilated by $\rho^{n+1}$ but such that $\rho^na_i\neq0$.
Take $a_i$ with bidegree $(n,n+1)$.
Again, it can be understood as the homotopy class of a map $a:S^{n+1,n+1}\to S^{1,0}\wedge X$.

On the other hand, the inclusion $S^{0,0}\hookrightarrow S^{n+1,n+1}$ induces a map in homology which corresponds to multiplication by $\rho^n$, and therefore $a$ factors through the cofiber $S^{n+1,n+1}/S^{0,0}\cong S^{1,0}\wedge (S_a^n)_+$ (isomorphism in the category of pointed $C_2$-spaces).
This is because of the choice of $a$, as $\rho^{n+1}a = 0$.
It is the linear extension of this map to $\F_2[S^{1,0}\wedge (S_a^n)_+]$ that is needed for the proof.
It will still be denoted by $a$.
In the structure theorem the factors $\Aop_n$ appear shifted by suspensions of the form $(r,0)$, but this only means that $a$ will have bidegree $(n+r,n+1)$ instead.

It remains to show that the map $a:\F_2[S^{1,0}\wedge (S_a^n)_+]\to \F_2[S^{1,0}\wedge X]$ so obtained induces a map $f:\F_2[(S_a^n)_+]\to \F_2[X]$.
This is achieved by applying the path-space functor $\Omega^{1,0}$: for any space $G$-space $Z$ and any $G$-representation $V$, $\Omega^V$ and $\F_2[Z]$
commute (cf.~\cite[10.4 Theorem]{mccord:classifying_spaces} or \cite[6.4.22 Theorem]{aguilar_et_al:algebraic_topology_homotopical_viewpoint}).
Hence
%
\[
f=\Omega^{1,0}a : \F_2[\Omega^{1,0}S^{1,0}\wedge (S_a^n)_+]\simeq \F_2[(S_a^n)_+] \longrightarrow \F_2[\Omega^{1,0}S^{1,0}\wedge X]\simeq \F_2[X].
\]
%

Finally, if
%
\[
H_{*,*}^{C_2}(X;\underline{F_2}) =  \left(\bigoplus_{i\in I} \Sigma^{p_i,q_i}\Mop_2\right) \oplus \left(\bigoplus_{j\in J} \Sigma^{r_j,0}\Aop_{n_j}\right),
%\oplus \left(\bigoplus_{j\in J} \Sigma^{r_j,0}A_{0}^*\right) 
\]
%
then the map
%%-----Diagram-------
%%\deactivatequoting
%\[
%\begin{tikzcd}[column sep=huge,row sep=huge]
%\left(\bigoplus_{i\in \tilde I} \tilde\F_2[S^{p_i,q_i}]\right) \oplus \left(\bigoplus_{j\in J} \tilde\F_2[S^{r_j}\wedge (S^0_a)_+]\right) \oplus \left(\bigoplus_{k\in K} \tilde\F_2[S^{r_k}\wedge (S^{n_k}_a)_+]\right) \arrow{rr}{\bigvee_{i\in I,j\in J,k\in K} (g_i\vee f_j \vee f_k)} & & \F_2[X],
%\end{tikzcd}
%\]
%%\activatequoting
%%-------------------
%
\begin{equation}
\left(\bigvee_{i\in I} g_i\right)\vee \left(\bigvee_{j\in J}f_j\right) : \left(\bigoplus_{i\in \tilde I} \tilde\F_2[S^{p_i,q_i}]\right) \oplus \left(\bigoplus_{j\in J} \tilde\F_2[S^{r_j}\wedge (S^{n_j}_a)_+]\right) \longrightarrow \F_2[X] ,
%\vee\left(\bigvee_{k\in K} f_k\right)   \oplus \left(\bigoplus_{j\in J} \tilde\F_2[S^{r_j}\wedge (S^0_a)_+]\right)
\label{eq:homotopy_zero-cycles}
\end{equation}
%
where the $g_i$ and $f_j$ are defined as explained above, provides the desired homotopy equivalence.
Moreover, as each of the factors is equivariant, so is their wedge product.
It is a group homomorphism by construction, as each of the maps $g_i,f_j$ is a linear extension of a map between spaces.

The map given in the statement is a representative of the homotopy inverse of \eqref{eq:homotopy_zero-cycles}, which can be chosen to be a group homomorphism.
\end{proof}

The next lemma will be used in the proof of Theorem \ref{thm:eilenberg-maclane_spaces}.

\begin{prop}
\label{prop:cycles_fixed_points}
Let $\{(X_n,Y_n)\}$ be a family of pairs, where $X_n$ is a topological Abelian group and $Y_n\subset X_n$ is a subgroup, endowed with the subspace topology.
Then, the following holds:
%
\[
\bigoplus_n X_n \bigg/ \bigoplus_n Y_n \cong \bigoplus_n X_n/Y_n.
\]
%
\end{prop}
\begin{proof}
This is true at the level of $\Z$-modules, but it must be checked that corresponding isomorphisms are continuous.
Let
%
\[
f: \bigoplus_n X_n \bigg/ \bigoplus_n Y_n \longrightarrow \bigoplus_n X_n/Y_n.
\]
%
As it maps out of a quotient, it is enough to see whether its composition with the quotient map $q:\bigoplus_n X_n\to \bigoplus X_n\bigg/\bigoplus_n Y_n$ is continuous.
Furthermore, as $qf$ maps out of a coproduct, it suffices to check that each $i_mqf$ is continous.
This composite map is simply
%
\[
x_m \longmapsto (\delta_{nm}x_m+Y_n)_n,
\]
%
which factors through the quotient map $q_m:X_m\to X_m/Y_m$ via the inclusion $\bar{i}_m:X_m/Y_m\to \bigoplus_n X_n/Y_n$:
%-----Diagram-------
%\deactivatequoting
\[
\begin{tikzcd}[column sep=huge,row sep=huge]
X_m \arrow{r}{i_mqf} \arrow{d}[swap]{q_m} & \displaystyle  \bigoplus_n X_n/Y_n \\
X_m/Y_m \arrow{ru}[swap]{\bar i_m} &
\end{tikzcd}
\]
%\activatequoting
%-------------------
As both are continuous, so is $i_mqf$.

For the opposite direction, if
%
\[
g: \bigoplus_n X_n/Y_n  \longrightarrow  \bigoplus_n X_n \bigg/ \bigoplus_n Y_n ,
\]
%
then it is enough to check on the map $q_m\bar{i}_mg$, which factors through the inclusion $i_m$ via $q$:
%-----Diagram-------
%\deactivatequoting
\[
\begin{tikzcd}[column sep=huge,row sep=huge]
X_m \arrow{r}{q_m} \arrow{d}[swap]{i_m} & X_m/Y_m \arrow{r}{\bar{i}_m} & \displaystyle \bigoplus_n X_n/Y_n \arrow{r}{g} & \displaystyle \bigoplus_n X_n\bigg/\bigoplus_n Y_n \\
 \displaystyle\bigoplus_n X_n \arrow{rrru}[swap]{q} & &
\end{tikzcd}
\]
%\activatequoting
%-------------------
\end{proof}

\begin{cor}
\label{cor:cycles_fixed_points}
Let $X$ be a $C_2$-space and let $\{Y_n\}_n$ be a family of topological $C_2$-spaces.
Suppose that
%
\[
\F_2[X]\cong \bigoplus_n \F_2[Y_n].
\]
%
Then
%
\[
\F_2[X^{C_2}]\cong \bigoplus_n \F_2[Y_n^{C_2}].
\]
%
A similar statement holds for the reduced case.
\end{cor}
\begin{proof}
It is easy to see that, for a $C_2$-space $Z$,
%
\[
\F_2[Z^{C_2}]\cong \left(\F_2[Z]\right)^{C_2}\Big/\im \big\{\id+\sigma\big\}.
\]
%
Hence, the result follows form the previous proposition.
\end{proof}


%\begin{rem}
%\label{rem:0-cycles}
%For the purposes of the next section, it is convenient to make a distinction between $S_a^0$ and $S_a^n$, $n>0$.
%Hence, it will be assumed that
%%
%\begin{equation}
%H_{C_2}^{*,*}(X;\underline{\F_2}) = \left(\bigoplus_{i\in I} \Sigma^{p_i,q_i}M_2\right) \oplus \left(\bigoplus_{j\in J} \Sigma^{r_k,0}A_{0}\right) \oplus \left(\bigoplus_{k\in K} \Sigma^{r_j,0}A_{n_k}\right),
%\label{eq:structure_theorem}
%\end{equation}
%%
%so that
%\begin{equation}
%\F_2[X] \simeq_{C_2} \left(\bigoplus_{i\in \tilde I} \tilde\F_2[S^{p_i,q_i}]\right) \oplus \left(\bigoplus_{j\in J} \tilde\F_2[S^{r_j}\wedge (S^0_a)_+]\right)  \oplus \left(\bigoplus_{k\in J} \tilde\F_2[S^{r_k}\wedge (S^{n_k}_a)_+]\right) .
%%
%\label{eq:0-cycles}
%\end{equation}
%%
%If, moreover, $X$ is a pointed space, then it has a fixed point and there exists $i\in I$ such that $(p_i,q_i)=(0,0)$:
%the set $\tilde I$ will denote the set $I$ with such an index $i$ removed.
%\end{rem}


\begin{thm}[Dold--Thom]
\label{thm:dold-thom}
\ \begin{enumerate}

\item (Classical statement, \cite{mccord:classifying_spaces}). Let $X$ be a based CW-complex and let $\Gamma$ be an Abelian group.
Then, for each $n\geq 0$ there is an isomorphism of groups
%
\[
\tilde{H}^n(X;M) \cong \pi(\tilde{\Gamma}[X]).
\]
%

\item (Equivariant statement, \cite{pedro:equivariant_dold-thom_theorem}). Let $G$ be a finite group and $M$ a discrete $\Z[G]$-module.
Let $X$ be a based $G$-CW-complex and let $V$ be a finite-dimensional
$G$-representation, then $M[X]$ is an equivariant infinite loop space and there is a natural equivalence
%
\[
\tilde{H}_{V}^G(X;\underline{M}) \cong \pi_V^G (M[X]).
\]
%
\end{enumerate}
\end{thm}

%-----------------------------------------------------------------------------------------------------------------------------------------------
%
%	SYMMETRIC PRODUCTS AND THEIR EQUIVARIANT HOMOLOGY %AND THE HOMOLOGY OF EQUIVARIANT EILENBERG-MACLANE SPACES
%
%-----------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Symmetric products and their equivariant homology}% of equivariant Eilenberg--MacLane spaces}
\label{subsec:symmetric_products}

Let $(X,x_0)$ be a pointed space (without an action) and let $(SP_nX,\ast_n)$ denote its $n$-fold symmetric product: $SP_nX$ is the quotient of the Cartesian product $X^n$ by the action of the symmetric group $\mathfrak S_n$.
We will use polynomial notation to represent the element: the equivalence class of a point $(x_1,\dots,x_n)$ will be denoted by the monomial $x_1\cdots x_n$.
Hence, $SP_nX$ can be regarded as the set of all monomials in $X$ of degree $n$.

For $m\leq n$, the space $SP_mX$ lies canonically inside $SP_nX$ as pointed spaces, via the inclusion
%
\[
%i_{m,n}(x_1,\dots,x_m\} = \{\underbrace{x_0,\dots,x_0}_{\text{$n-m$ times}},x_1,\dots,x_m\}.
i_{m,n}(x_1\cdots x_m)=x_0^{n-m}x_1\cdots x_m.
\]
%
Moreover, with this identification, $SP_nX$ is closed in $SP_{n+1}X$, so one can define the union
%
\[
SP_\infty X = \bigcup_n SP_n 
\]
%
with the customary conventions $SP_0X\equiv \{pt\}$ and $SP_1X\equiv X$.

Nakaoka proved in \cite{nakaoka:cohomology_symmetric_products} that the induced map in cohomology by $i_{m,n}$, admits a section, that is, there exists a homomorphism $s_{m,n}:H_{sing}^*(SP_mX;A)\to H_{sing}^*(SP_nX;A)$ such that the composition $s_{m,n}i_{m,n}^*$ is the corresponding identity on $H_{sing}^*(SP_mX;A)$.
In this fashion one can think of the cohomology group of $SP_mX$ as a subgroup of $H_{sing}^*(SP_nX;A)$.
It is this construction that leads to the results about the decomposition theorems for the cohomology of $SP_\infty X$ proved by Steenrod in \cite{steenrod:symmetric_products} (see also \cite{nakaoka:cohomology_spheres_modp}).
It is worth mentioning that the homomorphism $s_{m,n}$ only exists at the cohomology level and it is not induced by any map between spaces.

For the case when $(X,x_0)$ is $G$-space, the inclusion $i_{m,n}$ becomes equivariant (as base points are fix by convention), and so the above remains true.
Hence, one can try to adapt some of the reasoning made by Nakaoka when constructing such maps to the case of zero-cycles.
Fix $n\geq1$; it is enoguh to consider only the particular case $(n,n-1)$ for the general situation $(n,m)$, $m\leq n$, is done by composing the functions for the cases $(n,n-1)$, $(n-1,n-2)$,\dots, $(m+1,m)$.
Given another integer $m\leq n$, let $E_i^m:\F_2[SP_nX]\to \F_2[SP_mX]$ denote the $i$-th \emph{elementary symmetric function} on $\F_2[SP_mX]$, $1\leq i\leq m$:
%
\begin{align*}
%E_0^m\{x_1,\dots,x_n\}&=\{\underbrace{x_0,\dots,x_0}_{\text{$m$ times}}\} \\
E_0^m(x_1\cdots x_n)= x_0^m \\
E_1^m(x_1\cdots x_n)&=\sum_{i=1}^n x_0^{m-1}x_i \\
E_2^m(x_1\cdots x_n)&=\sum_{\substack{\text{$i,j=1$}\\ \text{$i<j$}}}^n x_0^{m-2}x_{i}x_{j} \\
&\vdots \\
E_m^m(x_1\cdots x_n) &= \sum_{\substack{\text{$i_1,\dots,i_m=1$} \\ \text{$i_1<i_2<\dots<i_m$}}}^n x_{i_1}\cdots x_{i_m}
\end{align*}
%
and extended linearly on general zero-cycles (notice that $E_n^n$ is the identity).
To simplify the notation let $E_i$ denote $E_i^{n-1}$
Now define $r\equiv r_{n,n-1}:\F_2[SP_{n}X]\to\F_2[SP_{n-1}X]$ by
%
\begin{equation}
%\begin{split}
r(x_1\cdots x_{n}) = \sum_{i=0}^{n-1} E_i(x_1\cdots x_n) = E_0(x_1\cdots x_n) +\dots + E_{n-1}(x_1\cdots x_n).
%\end{split}
\label{eq:retraction}
\end{equation}
%

\begin{rem}
\label{rem:retraction}
The space of zero-cycles $\F_2[SP_nX]$ is easily identified with the set of homogenous polynomials of degree $n$ with indeterminacies in the underlying set of the space $X$ and coefficients in $\F_2$.

Let $e_i$ be the \emph{$i$-th elementary symmetric polynomial function}:
%
\begin{align*}
e_0(x_1,\dots,x_n)&=1 \\
e_1(x_1,\dots,x_n)&=\sum_{i=1}^n x_i = x_1+\dots +x_n \\
e_2(x_1,\dots,x_n)&= \sum_{\substack{\text{$i,j=1$} \\ \text{$i<j$}}}^n x_ix_j = x_1x_2+x_1x_3+\dots+ x_{n-1}x_n \\ 
&\;\vdots \\
e_n(x_1,\dots,x_n) &= x_1x_2\cdots,x_n.
\end{align*}
%
Then the retraction $r$ has an expression in terms of this elementary polynomials:
%
\[
r(x_1\cdots x_n) = \sum_{i=0}^{n-1}x_0^{n-i}e_i(x_1,\dots,x_n) = x_0^n + x_0(x_1+\dots+x_n) + \cdots
\]
%
\end{rem}

\begin{prop}
%\label{prop:}
The map $r$ just introduced in \eqref{eq:retraction} continuous.
Furthermore, it is a retraction of the inclusion $i\equiv i_{n-1,n}:\F_2[SP_{n-1} X]\to \F_2[SP_{n} X]$, i.e. the composition $ir$ is the identity on $\F_2[SP_{n-1} X]$.
\end{prop}
\begin{proof}
To show that $r$ is continuous, it suffices to consider the covering map $\bar r:\F_2[X^{n}]\to \F_2[X^{n-1}]$ given by
%
\begin{equation}
%\begin{split}
\bar r(x_1,\dots x_{n}) = \sum_{i=1}^{n-1} \bar{E}_i(x_1,\dots, x_n) = \bar{E}_0(x_1,\dots, x_n) +\dots + \bar{E}_{n-1}(x_1,\dots, x_n)
%\end{split}
%\label{eq:retraction}
\end{equation}
%
This is continuous, for it is a linear combination of the lifted elementary symmetric functions $\bar E_i$, which are continuous themselves, being sums of projections $\proj_{i_1,\dots,i_k}:\F_2[X^{n}]\to \F_2[X^{k}]$, $(x_1,\dots,x_{n})\mapsto (x_{i_1},\dots,i_k)$, composed with inclusions $\bar{i}_k:\F_2[X^k]\to\F_2[X^{n-1}]$.

The second part is a consequence of the properties of these elementary symmetric polynomials.
Indeed,
%
\begin{equation*}
e_i(x_1,\dots, x_n) = e_i(x_1,\dots, \hat{x}_j,\dots x_n) + x_j e_{i-1}(x_1,\cdots, \hat{x}_j,\dots, x_n)
\end{equation*}
%
whenever $i>0$ (cf.~\cite{eisinberg&fedele:elementary_symmetric_functions}).
Hence:
%
\begin{equation*}
\begin{split}
r(x_0x_1\cdots x_{n-1})&= \sum_{i=1}^{n-1} x_0^{n-i}e_i(x_0,x_1,\cdots,x_{n-1}) + x_0^n =\\
&= \sum_{i=1}^{n-1} x_0^{n-i}e_i(x_1,\dots, x_{n-1}) +\sum_{i=1}^{n-1} x_0^{n-i}e_{i-1}(x_1,\dots x_{n-1})  + x_0^n = \\
&= x_0^{n-1} e_1(x_1,\dots, x_{n-1}) + x_0^n e_0(x_1,\dots, x_{n-1})+ x_0^n + \\
&+ x_0^{n-2} e_2(x_1,\dots, x_{n-1}) + x_0^{n-1} e_1(x_1,\dots, x_{n-1}) + \dots+ \\
&+x_0^2 e_{n-2}(x_1,\dots, x_{n-1}) + x_0^3 e_{n-3}(x_1,\dots, x_{n-1}) + \\
&+ x_0 e_{n-1}(x_1,\dots, x_{n-1}) + x_0^2 e_{n-2}(x_1,\dots, x_{n-1})  \equiv x_0x_1\dots x_{n-1} \pmod{2}.
\end{split}
\end{equation*}
%
\end{proof}


The existence of the retraction $r$ makes the short exact sequence
%
\[
0 \longrightarrow \tilde{\F}_2[SP_{n}X] \overset{i}{\longrightarrow} \tilde{\F}_2[SP_{n+1}X] \longrightarrow \tilde{\F}_2[SP_{n+1}X]\Big/ \tilde{\F}_2[SP_{n}X]\cong \tilde{\F}_2[SP_{n+1}X/SP_{n}X]\longrightarrow 0
\]
%
split, so that
%
\begin{equation}
\tilde{\F}_2[SP_{n+1}X] \cong \tilde{\F}_2[SP_{n}X]\oplus \tilde{\F}_2[SP_{n+1}X/SP_{n}X] 
\label{eq:0-cycles_split}
\end{equation}
%
as topological groups.

Notice that the split is equivariant with respect to the induced action of $C_2$.
The following result shows the advantage of this procedure.

\begin{prop}
\label{prop:free_homology}
The following hold:
\ \begin{enumerate}[ref=(\arabic*)]

\item $\displaystyle\tilde{H}_{*,*}^{C_2}(SP_nX;\underline{\F}_2) \cong \bigoplus_{k=0}^{n-1}\tilde{H}_{*,*}^{C_2}(SP_{k+1}X/SP_kX;\underline{\F}_2)$.

\item $\displaystyle \tilde{H}_{C_2}^{*,*}(SP_nX;\underline{F_2})\cong \bigoplus_{k=0}^{n-1} \tilde {H}_{C_2}^{*,*}(SP_{k+1}X/SP_kX;\underline{\F_2})$.

\item $\displaystyle \tilde{H}_{Bor}^*(SP_n X;\F_2)\cong \bigoplus_{k=0}^{n-1} \tilde{H}_{Bor}^*(SP_{k+1}X/SP_kX;\F_2)$.

\end{enumerate}
\end{prop}
\begin{proof}
For the results about bigraded homology, it is enough to apply the equviariant version of the Dold--Thom theorem given in Theorem \ref{thm:dold-thom} to \eqref{eq:0-cycles_split} and use induction.


In cohomology, start by identifying
%
\[
\tilde{H}_{C_2}^{p,q}(Y;\F_2) = \left[Y,\tilde{\F}_2[S^{p,q}]\right]
\]
%
so that an element $u\in \tilde{H}_{C_2}^{p,q}$ is regarded as the homotopy class of a map $u:SP_mX \to\tilde{\F}_2[S^{p,q}]$.
For such a map, there is an extension $\tilde{u}:\tilde{\F_2}[SP_m]\to\tilde{\F}_2[S^{p,q}]$ defined as follows:
%
\[
\tilde{u}(\{x_1,\dots,x_m\}+\dots+\{x_1',\dots,x_m'\}) = u\{x_1,\dots,x_m\} +\dots+ u\{x_1',\dots,x_m'\}.
\]
%
Then, $s$ can be defined as a composite in the following diagram:
%-----Diagram-------
%\deactivatequoting
\[
\begin{tikzcd}[column sep=huge,row sep=huge]
\F_2[SP_nX] \arrow{r}{r} & \F_2[SP_{n-1}X] \arrow[dashed]{r}{\tilde u} & \F_2[S^{p,q}] \\
SP_nX \arrow[hook]{u} & SP_{n-1}X \arrow[hook] {u}\arrow{ru}[swap]{u} &
\end{tikzcd}
\]
%\activatequoting
%-------------------
that is
%
\[
s(u)\{x_1,\dots,x_n\} = \tilde u(r\{x_1,\dots,x_n\}).
\]
%

An alternative proof is presented in Remark \ref{rem:free_cohomology} using the duality between homology and cohomology.

The proof for Borel cohomology is analogous, now considering
%
\[
\tilde{H}_{Bor}^q(Y;\F_2) = \left[Y\times_{C_2}EC_2,\tilde{\F}_2[S^q]\right].
\]
%
and the diagram
%-----Diagram-------
%\deactivatequoting
\[
\begin{tikzcd}[column sep=huge,row sep=huge]
\F_2[SP_nX]\times_{C_2}EC_2 \arrow{r}{r\times\id} & \F_2[SP_{n-1}X]\times_{C_2}EC_2 \arrow[dashed]{r}{\tilde u} & \F_2[S^q] \\
SP_nX\times_{C_2} EC_2  \arrow[hook]{u} & SP_{n-1}X\times_{C_2} EC_2 \arrow[hook] {u}\arrow{ru}[swap]{u} &
\end{tikzcd}
\]
%\activatequoting
%-------------------
where $\tilde{u}$ is the extension given by
%
\[
\tilde{u}[\{x_1,\dots,x_m\}+\dots+\{x_1',\dots,x_m'\},e] = u[\{x_1,\dots,x_m\},e] +\dots+ u[\{x_1',\dots,x_m'\},e].
\]
%

One may then define a section $s:H_{Bor}^{*}(SP_{n}X;\F_2)\to H_{Bor}^*(SP_{n+1}X;\F_2)$ of $i^*$ by repeating the construction of $r$, but now point-wise.
%For $q\geq 0$ and $[u]\in H_{Bor}^q(SP_nX;\F_2)$ a homotopy class, $u:SP_nX\times_{C_2}EC_2\to\tilde{\F}_2[S^q]$, $s[u]$ is the equivalence class of the map
%%
%\begin{equation*}
%\begin{split}
%s(u)[\{x_1,\dots,x_{n+1}\},e]  = &\sum_{1\leq i_1<\dots<i_n\leq n+1} u[\{x_{i_1},\dots,x_{i_{n}}\},e] + \\
%&+\sum_{1\leq i_1<\cdots<i_{n-1}\leq n+1}u[\{x_{i_1},\dots,x_{i_{n-1}},x_0\},e] +\dots+ \\
%&+ \sum_{1\leq i \leq n+1}^n u[\{x_i,x_0,\dots,x_0\},e] + u[\{x_0,\dots,x_0\},e].
%\end{split}
%\end{equation*}
%%


%Now $s:\tilde{H}_{Bor}^*(SP_{n-1}X;\F_2)\to \tilde{H}_{Bor}^*(SP_nX;\F_2)$, and acts on the element $[u]$ defined by $u:SP_mX\times_{C_2}EC_2\to\tilde{\F}_2[S^q]$ by considering the homotopy class of the map
%%
%\[
%s(u)[\{x_1,\dots,x_n\},e] = \sum_{k=0}^{n-2} \left(g_{n-1-k,n}(i_{n-1-k,n-1}u)\right)[\{x_1,\dots,x_n\},e] + u[\{x_0,\dots,x_0\},e].
%\]

\end{proof}

Since homology commutes with colimits, the previous result also implies the following:

\begin{cor}
%\label{cor:free_homology}
$\displaystyle\tilde{H}_{*,*}^{C_2}(SP_\infty X;\underline{\F}_2) \cong \bigoplus_{k=0}^{\infty}\tilde{H}_{*,*}^{C_2}(SP_{k+1}X/SP_kX;\underline{\F}_2)$.
\end{cor}


%-----------------------------------------------------------------------------------------------------------------------------------------------
%
%	THE COHOMOLOGY OF EQUVIARIANT EILENBERG--MACLANE SPACES
%
%-----------------------------------------------------------------------------------------------------------------------------------------------
\subsection{The cohomology of equivariant Eilenberg--MacLane spaces}
\label{subsec:cohomology}

Proposition \ref{prop:free_homology} provides a decomposition theorem similar to that of Steenrod in \cite{steenrod:symmetric_products} for the equivariant homology of the infinite symmetric product.
However, in order to state the freeness result about cohomology, it is necessary to retrieve the latter from the former using a similar relation to that of \eqref{eq:homology_dual_cohomology}.
In fact, it is the case that bigraded cohomology is dual to homology, in the following sense.

Therefore, the bigraded homology of a point possesses the structure of a ring, and the equivariant homology of a $C_2$-space becomes a module over this ring. 

This ring structure on $\Mop_2$ can be described as follows: by identifying $\M_2^{op}$ with $\Mop_2$, any element of $\Mop_2$ is characterised by its action on $1\in \M_2^{0,0}$; then, if $m,m'\in \Mop_2$ are homogenous elements with $m(1)=\mu$, $m'(1)=\mu'$, $\mu,\mu'\in \M_2$, their product is
%
\[
m\cdot m' = \mu' m = \mu m',
\]
%
where the product by scalars is defined with respect to the natural $\M_2$-module structure of $\Mop_2$.
This is equivalent to setting
%
\[
(m\cdot m')(1)=\mu\mu'.
\]
%
(i.e.~$m_\mu\cdot m_{\mu'}=m_{\mu\mu'}$).
%There are there are three distinguished elements: $m_\rho\in(\M_2^*)_{-1,-1}$, $m_\tau\in(\M_2^*)_{0,-1}$ and $m_{\theta}\in(\M_2^*)_{0,2}$, given by
%%
%\[
%m_{\rho}(1)=\rho, \qquad m_{\tau}(1)= \tau, \qquad  m_{\theta}(1)=\theta.
%\]
%%
Notice that this multiplicative law is \emph{not} induced by that of $\M_2$ taken point-wise.


%As $\Mop_2$ is the opposite module of $\M_2$, a ring structure on $\Mop_2$ exists, turning it into a graded ring such that equivariant homology becomes a graded module over it and the above isomorphism also exists in the category $\Mod_{\Mop_2}$.
%It is defined as follows: as it was said before, any element of $\Mop_2$ is characterised by its action on $1\in \M_2^{0,0}$; then, if $m,m'\in \Mop_2$ are homogenous elements with $m(1)=\mu$, $m'(1)=\mu'$, $\mu,\mu'\in \M_2$, their product is
%
%\[
%m\cdot m' = \mu' m = \mu m',
%\]
%%
%where the product by scalars is defined with respect to the natural $\M_2$-module structure of $\Mop_2$.
%This is equivalent to setting
%%
%\[
%(m\cdot m')(1)=\mu\mu'.
%\]
%%
%(i.e. $m_\mu\cdot m_{\mu'}=m_{\mu\mu'}$).

\begin{rem}
%\label{rem:}
Given the bigraded ring $\M_2$, consider the \emph{opposite ring} $\M_2^{op}$:
%
\[
\left(\M_2^{op}\right)_{p,q} = \M_2^{-p,-q}
\]
%
with usual addition and multiplication.
Then $\M_2^{op}\cong \Mop_2$ as bigraded rings and, when regarded as modules over $\M_2$, $\M_2^{op}\cong \Mop_2$.%, as Lemma \ref{lem:duals} shows.
%Because of this, no distinction between $\Mop_2$ and $\M_2^{op}$ will be made, identifying $\M_2^{op}$ with $\Mop_2$.
\end{rem}

Because $\Mop_2$ is a ring, one can consider the dual module of $H_{*,*}^{C_2}(X;\underline{\F_2})$.
For $X=pt,S_a^n$ one has:
%
\[
\left(({\Mop_2})^{\op}\right)^{p,q} = \Hom_{\Mop_2}\big(\Mop_2,\Sigma^{p,q} \Mop_2\big)
\]
%
and
%
\[
\left(({\Aop_n})^{\op}\right)^{p,q} = \Hom_{\Mop_2}\big(\Aop_n,\Sigma^{p,q} \Mop_2\big),
\]
%
respectively.
Then $({\Mop_2})^{^\op}\cong \M_2$ and $({\Aop_n})^{^\op}\cong \A_n$ as bigraded $\M_2$-modules.%, as one can prove using the same arguments of Lemma \ref{lem:duals}.
Furthermore, as $\Mop_2$ is the opposite ring of $\M_2$, self-injectivity is preserved, and one recovers the bigraded cohomology groups of the space by taking the dual: 

%With this conventions, $\Mop_2$ is a commutative ring with unit and homology becomes an $\Mop_2$-module.
%Furthermore, one can recover $\RO(C_2)$-graded cohomology from homology as before:
%
\begin{prop}
%\label{prop:}
For each $C_2$-space $X$, the following is an isomorphism of $\M_2$-modules:
\begin{equation*}
H_{C_2}^{p,q}(X;\underline{\F_2}) \cong \Hom_{\Mop_2}\left(H_{*,*}^{C_2}(X;\underline{\F_2}),\Sigma^{p,q}\Mop_2\right) .
\label{eq:cohomology_dual_homology}
\end{equation*}
\end{prop}
\begin{proof}
The assignment
%
\[
X\longmapsto \Hom_{\Mop_2}(H_{*,*}^{C_2}(X;\underline{\F_2}),\Sigma^{*,*}\Mop)
\]
%
defines a family of contravariant functors that we shall denote by $E^{*,*}$ from the category of topological spaces into the category of Abelian groups.
Along with the groups, a theory like this needs suspension isomorphisms
$\sigma^W:E^V(X)\to E^{V\oplus W}(\Sigma^W X)$ for every $C_2$-representation $W$.
We define them as the pullbacks of the suspension isomorphisms
%
\[
\rho_W:H_{V\oplus W}^{C_2}(\Sigma^W X; \underline{\F_2})\longrightarrow H_V^{C_2}(X;\underline{\F_2})
\]
%
that Bredon homology possesses.

We show that $E^{*,*}$, together with the suspension isomorphisms $\{\sigma^W\}$ so defined, satisfies the axioms for a bigraded cohomology theory (cf.~\cite[Chaper XIII]{MayJP96}):
\begin{enumerate}

\item \emph{Homotopy axiom}. Clearly, if $f,g:X\to Y$ are homotopic, then $E^{*,*}(f)=E^{*,*}(g)$.

\item \emph{Additivity}. Let $\{X_i\}$ be a family of topological spaces.
Then
%
\[
E^{*,*}(\vee_i X_i) \cong \prod_i E^{*,*}(X_i)
\]
%
due to the properties of the functor $\Hom$ and the additivity axiom for homology.
%%
%\begin{equation*}
%\begin{split}
%\Hom_{\Mop_2}\left(H_{*,*}^{C_2}(\vee_n X_n;\underline{\F_2}),\Sigma^{p,q}\Mop_2\right) &\cong %\Hom_{\Mop_2}\left(\bigoplus_n H_{*,*}^{C_2}(X_n;\underline{\F_2}),\Sigma^{p,q}\Mop_2\right) \cong \\
%&\cong \prod_n\Hom_{\Mop_2}\left(H_{*,*}^{C_2}X_n;\underline{\F_2}),\Sigma^{p,q}\Mop_2\right) 
%\end{split}
%\end{equation*}
%%

\item \emph{Transitivity of the suspensions}. Let $V$, $W$, $W'$ and $Z$ be representations of $C_2$ and let $\alpha:W\to W'$.
Then the following diagrams commute:
%-----Diagram-------
%\deactivatequoting
\[
\begin{tikzcd}[column sep=huge,row sep=huge]
E^V(X) \arrow{rr}{\sigma^W} \arrow{rd}[swap]{\sigma^{W\oplus Z}} & & E^{V\oplus W}(\Sigma^WX) \arrow{ld}{\sigma^Z} \\ 
& E^{V\oplus W\oplus Z}(\Sigma^{W\oplus Z}X) &
\end{tikzcd}
\]
%\activatequoting
%-------------------
and
%-----Diagram-------
%\deactivatequoting
\[
\begin{tikzcd}[column sep=huge,row sep=huge]
E^V(X) \arrow{r}{\sigma^W} \arrow{d}[swap]{\sigma^{W'}} & E^{V\oplus W}(\Sigma^W X) \arrow{d}{E^{\id\oplus\alpha}(\id_{\Sigma^W X})} \\
E^{V\oplus W'}(\Sigma^{W'}X) \arrow{r}[swap]{E^{*,*}(\Sigma^\alpha\id_X)} & E^{V\oplus W'}(\Sigma^W X).
\end{tikzcd}
\]
%\activatequoting
%-------------------


\item \emph{Exactness}. Given a cofiber sequence $X\to Y\to Z$, homology provides a long exact sequence
%
\[
\cdots \longrightarrow H_{*,*}^{C_2}(X;\underline{\F_2}) \longrightarrow H_{*,*}^{C_2}(Y;\underline{\F_2}) \longrightarrow H_{*,*}^{C_2}(Z;\underline{\F_2}) \longrightarrow H_{*-1,*}^{C_2}(X;\underline{\F_2}) \longrightarrow \cdots
\]
%
As $\Mop_2$ is self-injective, $\Hom_{\Mop_2}(-,\Sigma^{*,*}\Mop_2)$ preserves exactness, and we obtain the corresponding long exact sequence
%
\[
\cdots \longrightarrow E^{*,*}(Z) \longrightarrow E^{*,*}(Y) \longrightarrow E^{*,*}(X) \longrightarrow E^{*+1,*}(Z) \longrightarrow \cdots
\]
%
\end{enumerate}
\end{proof}


\begin{rem}
\label{rem:free_cohomology}
This result provides an alternative proof for statement (2) in Proposition \ref{prop:free_homology}.
\end{rem}


%\begin{rem}
%%\label{rem:}
%Consider the category $\ROC\Rng$ whose objects are bigraded rings and whose morphisms are pairs $(f,\varphi)$, where $\varphi:\RO(C_2)\to\RO(C_2)$ is a group homomorphism and $f:R\to S$ is a ring homomorphism which is graded in the sense that $f(R^V)\subset S^{\varphi(V)}$ for all $V\in\RO(C_2)$.
%An isomorphism in $\ROC\Rng$ consists of a pair $(f,\varphi)$ where both $f$ and $\varphi$ are isomorphisms in the categories $\Rng$ and $\Ab$, respectively, and the former and its inverse are graded in the previous sense.
%Then $\M_2$ and $\Mop_2$ are isomorphic rings in $\ROC\Rng$.
%\end{rem}

Finally, a similar $\rho$-localisation theorem for homology holds.

\begin{prop}
\label{prop:localisation_homology}
Let $X$ be a finite $C_2$-CW complex. Then
%
\[
m_\rho^{-1}H^{C_2}_{*,*}(X;\underline{\F_2}) \cong H^{sing}_*(X^\sigma;\F_2)\otimes_{\F_2} m_\rho^{-1}\Mop_2
\]
%
as $m_\rho^{-1}\Mop_2$-modules.
\end{prop}


The following is proven by combining the results of Proposition \ref{prop:main_result}, Proposition \ref{prop:free_homology} and Theorem \ref{thm:gamma_products} .

\begin{thm}
\label{thm:eilenberg-maclane_spaces}
For any representation $V$ of $C_2$, the bigraded ordinary cohomology of the equivariant Eilenberg--MacLane space $K(\underline{\Z},V)=SP_\infty S^V$ with coefficients in the constant Mackey functor $\underline{\F_2}$ is free.
\end{thm}
\begin{proof}
It is first shown that the bigraded cohomology of each quotient $SP_{n+1}S^V/SP_nS^V$ is free.
Because it is a finite complex, it is enough to use Borel cohomology.
Then
%
\begin{equation}
H_{Bor}^*(SP_{n+1}S^V;\F_2) \cong H_{Bor}^*(SP_nS^V;\F_2) \oplus H_{Bor}^*(SP_{n+1}S^V/SP_nS^V;\F_2).
\label{eq:splitting_borel}
\end{equation}
%
As both $SP_{n+1}S^V$ and $SP_nS^V$ are maximal (cf.~Theorem \ref{thm:gamma_products}), Proposition \ref{prop:main_result_borel} implies that their Borel cohomology is.
Hence, \eqref{eq:splitting_borel} shows that the relative cohomology is a projective $\F_2[x]$-module.
But since $\F_2[x]$ is a principal ideal domain, it follows that $H_{Bor}^*(SP_{n+1}S^V/SP_nS^V;\F_2)$ is free, and this part is concluded.

Therefore, by Proposition \ref{prop:free_homology}, the bigraded homology of $SP_\infty X$ is free; write
%
\begin{equation}
H_{*,*}^{C_2}(SP_\infty S^V;\underline{\F_2}) = \bigoplus_{i\in I} \Sigma^{p_i,q_i}\Mop_2
\label{eq:free_equivariant_homology}
\end{equation}
%
for some indexing set $I$ and actual representations $(p_i,q_i)$.
As cohomology can be computed from homology by taking duals (cf.~\eqref{eq:cohomology_dual_homology}), the properties of the Hom functor directly leads to
the expression
%
\[
H_{C_2}^{*,*}(SP_\infty S^V;\underline{\F_2}) = \prod_{i\in I} \Sigma^{p_i,q_i}\M_2 .
\]
%

It remains to show that this is a direct sum, i.e.~for any element $(\mu_i)\in\prod_{i\in I}\Sigma^{p_i,q_i}\M_2$, only finitely many $\mu_i$ are non-zero.
For this purpose, it will first be shown that for each $n\in\N$, the cardinality of the set
%
\begin{equation}
I_n=\{i\in I \mid p_i-q_i = n\}
\label{eq:set}
\end{equation}
%
is finite.
\begin{comment}
\footnote{$\Rep(C_2)$-complexes are defined in \cite{clover_may:freeness_theorem_cohomology} as those complexes constructed by attaching cells of the form $D(\R^{p,q})$.
A finite such complex is a complex with (possibly infinitely many) cells $\{D(\R^{p_i,q_i})\}$ such that the cardinality of the set
%
\begin{equation}
I_n=\{i\mid p_i-q_i=n\}
\tag{\ref{eq:set}}
\end{equation}
%
is finite for every $n$.
Then, the authors show that their cohomology with coefficients $\underline{\F_2}$ is free.
Nevertheless, the finiteness of the sets $I_q$ does not immediately prove that $SP_\infty S^V$ is a finite $\Rep(C_2)$-complex, and therefore the results of \cite{clover_may:freeness_theorem_cohomology} do not apply.}.
\end{comment}

From \eqref{eq:free_equivariant_homology} and using the same reasoning as in Theorem \ref{thm:0-cycles}, there is a decomposition
%
\[
\tilde{\F}_2[SP_\infty S^V]\simeq \bigoplus_{n} \tilde{\F}_2[SP_{n+1}S^V/SP_nV];
\]
%
then Corollary \ref{cor:cycles_fixed_points} applied to this results in 
%
\[
\tilde{\F}_2[(SP_\infty S^V)^{C_2}]\simeq \bigoplus_{n} \tilde{\F}_2[(SP_{n+1}S^V/SP_nV)^{C_2}].
\]
%
Now, for a fixed integer $q>0$, the standard Dold--Thom theorem of Theorem \ref{thm:dold-thom} gives
%
\[
\tilde{H}_q^{sing}\left((SP_\infty S^V)^{C_2};\F_2\right) \cong \bigoplus_{n} \tilde{H}_q^{sing}\left((SP_{n+1}S^V/SP_n S^V)^{C_2};\F_2\right).
\]
%
Moreover, as the quotients are finite complexes, the homology of their fixed points can be computed by using Proposition \ref{prop:localisation_homology}, yielding the isomorphism
%
\[
\tilde{H}_q\left((SP_\infty S^V)^{C_2};\F_2\right) \cong \bigoplus_{I_q} \F_2,
\]
%
where $I_q$ is defined as in \eqref{eq:set} an may be an infinite set.

On the other hand, the space $\F_2[(SP_\infty S^V)^{C_2}]$ has the homotopy type of a product of ordinary Eilenberg--MacLane spaces $K(\Z,n_\alpha)$ satisfying the extra condition that, for each $n\in \N$, only finitely many indices $\alpha$ indexing such a product satisfy the relation $n_\alpha=n$ REFERENCE?.
As the integral homology of these spaces is finitely generated at each degree (c.f.~Lemma 1.10 in \cite[Chapter 1]{hatcher:spectral_sequences}), 
the homology of $\F_2[(SP_\infty S^V)^{C_2}]$ is also finite at each degree, by using Künneth theorem.
Thus the set $I_q$ must be finite for all $q$.

To complete the proof, it is convenient to regard $\M_2$ as the dual module of $\Mop_2$, so that an element $\mu_i$ becomes a homomorphism (denoted by the same symbol) $\mu_i:\Sigma^{p_i,q_i}\Mop_2\longrightarrow \Mop_2$.
More precisely, if
%
\[
(\mu_i)_i\in\left(\prod_{i\in I}\Sigma^{p_i,q_i}\M_2,\right)^{r,s},
\]
%
then
%
\[
\mu_i: \left(\Sigma^{p_i,q_i}\Mop_2\right)_{u,v}\longrightarrow \left(\Sigma^{r,s}\Mop_2\right)_{u,v} .
\]
%
Such an element is completely characterised by its value on the identity $\id_i\in(\Sigma^{p_i,q_i}\Mop_2)_{p_i,q_i}$:
%
\[
\mu_i(\id_i)\in \left(\Sigma^{r,s}\Mop_2\right)_{p_i,q_i}  = (\Mop_2)_{p_i-r,q_i-s}.
\]
%
As the difference $p_i-q_i\to\infty$ and each $(p_i,q_i)$ is an actual representation, only finitely many points $(p_i,q_i)$ are inside either of the cones of $\Sigma^{r,s}\Mop_2$.
Thus, $\mu_i\equiv 0$ for all but finitely many indices $i\in I$.
This is best seen in Figure \ref{fig:proof}.
\end{proof}

\begin{figure}[H]
     \centering
\begin{pspicture}(-4,-4)(4,4)
\psset{unit = 0.7}
    \psaxes[linewidth=.4pt,linecolor=gray,showorigin=false,ticks=none,labels=none]{->}(-5.5,-4.5)(-6,-5)(6,5)[$u$,0][$v$,90]
    \psline[linewidth=.7pt,linecolor=black]{->}(-1,-1)(4.5,4.5)
    \psline[linewidth=.7pt,linecolor=black]{->}(-1,-1)(-1,4.5)
    \psline[linewidth=.7pt,linecolor=black]{->}(-1,-2.5)(-1,-4.5)
    \psline[linewidth=.7pt,linecolor=black]{->}(-1,-2.5)(-2.5,-4.5)


    \uput[0](-1,-1.2){$(r,s+2)$}
    \uput[0](-1,-2.4){$(r,s)$}
    \uput[0](2.9,-0.5){$(p_i,q_i)$}
    \uput[0](-0.7,3.55){\tiny$u-v\leq r-s-2$}
    
    \pscircle[fillstyle=solid,fillcolor=black,dimen=inner](-1,-1){0.05}
    \pscircle[fillstyle=solid,fillcolor=black,dimen=inner](-1,-2.5){0.05}
    \pscircle[fillstyle=solid,fillcolor=black,dimen=inner](3,0){0.07}
    


\end{pspicture}
         \caption{\small Representation of $\Sigma^{r,s}\Mop_2$.
         As $p_i\geq r$, the only option for $\mu_i(\id_i)$ to be non-zero is to be within the upper cone.
         This region is described by the inequality $v-s-2\geq u-r$.
         But since $p_i-q_i\to\infty$ and $p_i\geq q_i\geq 0$, only finitely many pairs $(p_i,q_i)$ will be in there.}
         \label{fig:proof}
\end{figure}



\textcolor{red}{I suggest that we finish the paper with the following conjecture:}

One of the key aspects in the proof of this last theorem is that the generators $\mu_i$ of the free module $H_{*,*}^{C_2}(SP_\infty S^V;\underline{\F_2})$ satisfy the following condition (cf.~display \eqref{eq:set}): for each $n$, the set 
%
\[
\{\mu_i\mid \bideg \mu_i=(p_i,q_i) \mbox{ and } p_i-q_i= n\}
\]

is finite.
This fact suggests that the infinite symmetric products of a representation sphere, and more generally infinite symmetric products of $\Rep(C_2)$-complexes of finite type are also $\Rep(C_2)$-complexes of finite type.

These complexes have been recently studied by Hogle and May in \cite{clover_may:freeness_theorem_cohomology}, where the authors obtained a complete characterisation of their cohomology.
The following are some of the main definitions regarding this family of complexes.

A \emph{$\Rep(G)$-complex} is a $G$-space $X$ with a filtration $X_n$, where $X_0$ is a disjoint union of trivial orbits of the form $G/G = \ast$ and $X_n$ is obtained from $X_{n-1}$ by attaching cells of the form $D(V_\alpha)$, where $V_\alpha$ is an $n$-dimensional real representation of $G$.
The cells are attached along maps $f_\alpha : S(V_\alpha) \to X_{n-1}$ via usual pushout diagrams.

In the case $G = C_2$, any finite-dimensional representation is of the form $\R^{p,q}$ for
certain integers $p$ and $q$ satisfying $p\geq q\geq 0$.
%The integer $p$ is called the topological dimension while $q$ is the weight.
A $\Rep(C_2)$-complex of \emph{finite type} is a complex that has finitely many cells of
each fixed-set dimension: for each $n \geq 0$, there are finitely many cells $e_\alpha$ which are of
the form $D(\R^{p_\alpha,q_\alpha})$ with $p_\alpha - q_\alpha = n$.

The following is one of the main results in \cite{clover_may:freeness_theorem_cohomology}:

\begin{thm}
The bigraded Bredon cohomology of a $\Rep(C_2)$-complex of finite type is free.
\end{thm}

Based on the proof of Theorem \ref{thm:eilenberg-maclane_spaces} and the previous theorem of Hogle and May we conjecture the following:

\begin{conj}
The symmetric powers of a $\Rep(C_2)$-complex are $\Rep(C_2)$-complexes.
Moreover, if it is of finite type, then so are all of its symmetric products.
In particular, the equivariant Eilenberg--MacLane spaces $K(\underline{\Z},V)$ are $\Rep(C_2)$-complexes of finite type.
\end{conj}
